Stellar and dark matter density in the Local Universe

We calculate the mean density profiles for luminous and dark matter on distance scales $D \sim(1 - 100)$ Mpc around us using recent all-sky catalogs of galaxy groups. Within the Local Volume $( D < 11 ~\rm Mpc)$ we derived the mean stellar density $\Omega_*= 0.44\%$ in the critical density units and the mean total matter density $\Omega_m = 0.17$. In the sphere with a radius of 40 Mpc these quantities drop to $\Omega_* = 0.24 - 0.32\%$ and $\Omega_m = 0.09 - 0.14$. In a larger volume within $D\sim135$ Mpc the discussed densities become more uncertain: $\Omega_* = 0.20 - 0.24\%$ and $\Omega_m = 0.05 - 0.16$. We summarize that the major part of the cosmic dark matter locates outside the virial and collapsing zones of groups and clusters.

==> journals1.tex <==
\def\apj{Astrophys. J.\ }
\def\apjl{Astrophys. J. Lett.\ }
\def\apjs{Astroph. J. Suppl. Ser.\ }
\def\mnras{Mon. Not. R. Astron. Soc.\ }
%\def\nat{Nature}
\def\aap{Astron. Astrophys.\ }
%\def\pr{Phys. Rev.}
%\def\pra{Phys. Rev. {\rm A}}
%\def\prc{Phys. Rev. {\rm C}}
%\def\prb{Phys. Rev. {\rm B}}
\def\prd{Phys. Rev. {\rm D}\ }
%\def\prl{Phys. Rev. Lett.}
%\def\plb{Physics Letters {\rm B}}
\def\apss{Astroph. Space Sci.\ }
\def\pla{Phys. Lett. A\ }
\def\ssr{Space Sci. Rev.\ }
\def\araa{Ann. Rev. Astron. Astrophys.\ }
\def\aj{Astron. J.\ }
\def\jphys{J. Phys.\ }
\def\npa{Nucl. Phys. A\ }
\def\npb{Nucl. Phys.  B\ }
\def\ijmpe{Int. J. Mod. Phys. E\ }
\def\ijmpd{Int. J. Mod. Phys. D\ }
\def\ijmpa{Int. J. Mod. Phys. A\ }
\def\pasj{Proc. Astron. Soc. Japan\ }
